First results on FHM -- a Floating Hole Multiplier

A proof of principle of a novel concept for event recording in dual-phase liquid xenon detectors -- the Floating Hole Multiplier (FHM) -- is presented. It is shown that a standard Thick Gaseous Electron Multiplier (THGEM), freely floating on the liquid xenon surface permits extraction of electrons from the liquid to the gas. Secondary scintillation induced by the extracted electrons in the THGEM holes as well as in the uniform field above it was observed. The first results with the FHM indicate that the concept of floating electrodes may offer new prospects for large-scale dual-phase detectors, for dark matter searches in particular.

==> src/dummy.tex <==
\section{Dummy section for unused material}
\label{sec:dummy}

This is a collection of unused or new material.

\begin{figure}
    \centering
    \includegraphics[width=7cm]{img/s1_integral.png} 
    \caption{\sone spectrum of alpha signals.\mynote{VC: Not sure we need this figure, but the mean should be consistent with other estimates!}}
    \label{fig:s1_integral}    
    % Data 23/05/2022 - p.206 wfms folder "floating/s2"
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{img/s2area_vs_vdrift.png} 
    \caption{\mynote{NOT USED} Variation of the area of S2 signals as a function of the drift field.}
    \label{fig:s2_area_vs_vdrift}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{img/drifttime_vs_vdrift.png} 
    \caption{\mynote{NOT USED} Variation of drift time as a function of the drift voltage for a fixed distance.}
    \label{fig:drifttime_vs_drift}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{img/s2_spectra.png} 
    \caption{\mynote{NOT USED} \stwo spectrum of alpha signals for $\vdrift = 400$ V/cm, $\dvthgem = 2.5$ kV and several values of \vextr \gonzalo{Switched to linear scale and lower number of voltages displayed.}}
    \label{fig:s2_spectra}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{img/60kev_spectra.png} 
    \caption{\mynote{NOT USED} \stwo spectra of 60 keV gamma signals for $\vdrift = 400$ V/cm, $\dvthgem = 2$ kV and several values of \vextr.}
    \label{fig:60kev_spectrum}
\end{figure}


